Sculpting Holistic 3D Representation in Contrastive Language-Image-3D Pre-training

Contrastive learning has emerged as a promising paradigm for 3D open-world understanding, i.e., aligning point cloud representation to image and text embedding space individually. In this paper, we introduce MixCon3D, a simple yet effective method aiming to sculpt holistic 3D representation in contrastive language-image-3D pre-training. In contrast to point cloud only, we develop the 3D object-level representation from complementary perspectives, e.g., multi-view rendered images with the point cloud. Then, MixCon3D performs language-3D contrastive learning, comprehensively depicting real-world 3D objects and bolstering text alignment. Additionally, we pioneer the first thorough investigation of various training recipes for the 3D contrastive learning paradigm, building a solid baseline with improved performance. Extensive experiments conducted on three representative benchmarks reveal that our method significantly improves over the baseline, surpassing the previous state-of-the-art performance on the challenging 1,156-category Objaverse-LVIS dataset by 5.7%. The versatility of MixCon3D is showcased in applications such as text-to-3D retrieval and point cloud captioning, further evidencing its efficacy in diverse scenarios. The code is available at https://github.com/UCSC-VLAA/MixCon3D.

==> experiments/tab_abl_inference.tex <==
\begin{wraptable}{r}{0.5\textwidth}
  % \vspace{-4pt}
%\begin{table*}[t]  
  \centering
  \caption{The analysis of cross-modal representation ensembing schemes in Objaverse-LVIS.}
  \renewcommand\tabcolsep{3pt} 
  \resizebox{1.0\linewidth}{!}{
  \begin{tabular}{ccc|cccccc}
    \toprule
    \multirow{2}*{\makecell[c]{Point \\  Cloud}} & \multirow{2}*{Image} & \multirow{2}*{\makecell[c]{Multi- \\  View}} & \multicolumn{4}{c}{\small Objaverse-LVIS}\\
    \cmidrule(lr){4-7}
    &  &  & Top1 & Top1-C & Top3 & Top5\\
    \midrule
    \checkmark    & \XSolidBrush & - & 50.4 & 37.4 & 72.2 & 79.1\\
    \XSolidBrush  & \checkmark   & - & 44.5 & 34.5 & 64.2 & 70.6\\
    \XSolidBrush  & \checkmark   & \checkmark & 51.9 & 38.5 & 73.1 & 79.4\\
    \checkmark    & \checkmark   & - & 51.6 & 37.6 & 73.4 & 80.1 \\
    \checkmark    & \checkmark   & \checkmark & \textbf{52.5} & \textbf{38.8} & \textbf{74.5} & \textbf{81.2} \\
    % \rowcolor{yellow!20}
    \bottomrule
  \end{tabular}
  }
  \label{tab:abl_inference}
\end{wraptable}

==> experiments/tab_abl_inference_arxiv.tex <==
\begin{table*}[t] 
\vspace{-.5em}
\label{tab:abla-mv_all}
\begin{subtable}[h]{0.33\textwidth}{
\centering
\caption{Variants of fusion $g^{MV}$}
\label{tab:abl_g_mv}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1mm}{
  \begin{tabular}{l|cccccccc}
    \toprule
    \multirow{2}*{\makecell[c]{Function $g^{MV}$}} & \multicolumn{2}{c}{\small O-LVIS} & \multicolumn{2}{c}{\small S-Object} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & Top1 & Top1-C & Top1 & Top1-C\\
    \midrule
    - & 51.6 & 38.2 & 58.1 & 61.9\\
    \rowcolor{blue!8} View-pooling & 52.5 & 38.8 & \textbf{58.6} & \textbf{62.3} \\
    View-pooling + FC & \textbf{52.7} & \textbf{39.1} & 52.4 & 54.1\\
    Max pooling & 52.1 & 38.4 & 56.7 & 60.0\\
    Max pooling + FC & 51.6 & 38.0 & 55.8 & 58.7\\
    % \rowcolor{yellow!20}
    \bottomrule
  \end{tabular}}
}}
\end{subtable}
\hfill
\begin{subtable}[h]{0.29\textwidth}
\centering
\caption{The amount of view}
\label{tab:abla_view_num}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1mm}{
  \begin{tabular}{c|cccccccc}
    \toprule
    \multirow{2}*{\makecell[c]{Multi-View}} & \multicolumn{2}{c}{\small O-LVIS} & \multicolumn{2}{c}{\small S-Object} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & Top1 & Top1-C & Top1 & Top1-C\\
    \midrule
     1 & 51.6 & 38.2 & 58.1 & 61.9 \\
     2 & 52.3 & 38.9 & 57.0 & 60.5 \\
     \rowcolor{blue!8} 4 & 52.5 & 38.8 & \textbf{58.6} & \textbf{62.3}\\
     8 & 52.7  & 39.3 & 58.1 & 61.7 \\
     12 & \textbf{53.2} & \textbf{39.5} & 54.2 & 56.1\\
    % \rowcolor{yellow!20}
    \bottomrule
  \end{tabular}
}
}
\end{subtable}
\hfill
\begin{subtable}[h]{0.32\textwidth}
\caption{Multi-Modal Inference}
\label{tab:abl_inference} % #num latent, use pt pos
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{1mm}{
  \begin{tabular}{ccc|cccccc}
    \toprule
    \multirow{2}*{\makecell[c]{Point \\  Cloud}} & \multirow{2}*{Image} & \multirow{2}*{\makecell[c]{Multi- \\  View}} & \multicolumn{4}{c}{\small Objaverse-LVIS}\\
    \cmidrule(lr){4-7}
    &  &  & Top1 & Top1-C & Top3 & Top5\\
    \midrule
    \checkmark    & \XSolidBrush & - & 50.4 & 37.4 & 72.2 & 79.1\\
    \XSolidBrush  & \checkmark   & - & 44.5 & 34.5 & 64.2 & 70.6\\
    \XSolidBrush  & \checkmark   & \checkmark & 51.9 & 38.5 & 73.1 & 79.4\\
    \checkmark    & \checkmark   & - & 51.6 & 37.6 & 73.4 & 80.1 \\
    \rowcolor{blue!8} \checkmark    & \checkmark   & \checkmark & \textbf{52.5} & \textbf{38.8} & \textbf{74.5} & \textbf{81.2} \\
    % \rowcolor{yellow!20}
    \bottomrule
  \end{tabular}
}
}
\end{subtable}
\caption{\yp{Ablation studies of multi-view mechanism and cross-modal representation ensembling schemes.} 
We report results on Objaverse-LVIS (O-LVIS) and ScanObjectNN (S-Object).}
\end{table*}
